VGGT-HPE: Reframing Head Pose Estimation as Relative Pose Prediction

Monocular head pose estimation is traditionally formulated as direct regression from a single image to an absolute pose. This paradigm forces the network to implicitly internalize a dataset-specific canonical reference frame. In this work, we argue that predicting the relative rigid transformation between two observed head configurations is a fundamentally easier and more robust formulation. We introduce VGGT-HPE, a relative head pose estimator built upon a general-purpose geometry foundation model. Finetuned exclusively on synthetic facial renderings, our method sidesteps the need for an implicit anchor by reducing the problem to estimating a geometric displacement from an explicitly provided anchor with a known pose. As a practical benefit, the relative formulation also allows the anchor to be chosen at test time - for instance, a near-neutral frame or a temporally adjacent one - so that the prediction difficulty can be controlled by the application. Despite zero real-world training data, VGGT-HPE achieves state-of-the-art results on the BIWI benchmark, outperforming established absolute regression methods trained on mixed and real datasets. Through controlled easy- and hard-pair benchmarks, we also systematically validate our core hypothesis: relative prediction is intrinsically more accurate than absolute regression, with the advantage scaling alongside the difficulty of the target pose. Project page and code: https://vasilikivas.github.io/VGGT-HPE

==> sec/1_intro_back.tex <==
\section{Introduction}
\label{sec:intro}

Head pose estimation — recovering the full 6DoF position and orientation of a human head from a single image — is a fundamental building block in computer vision. Accurate head pose drives a wide range of downstream applications, from gaze estimation and driver attention monitoring to sign language recognition, human-robot interaction, and augmented reality. Despite decades of progress, robust head pose estimation in unconstrained settings remains challenging due to appearance variability, partial occlusions, and the inherent ambiguity of monocular 3D inference.



The dominant paradigm in learned head pose estimation treats the problem as direct regression from a single image to an absolute pose vector — typically three Euler angles (yaw, pitch, roll) and, less commonly, a 3D translation. Methods such as HopeNet, 6DRepNet, and WHENet train deep networks to map face crops directly to global orientation, implicitly requiring the model to internalize a canonical reference frame from the training data. This formulation places a heavy burden on the network: it must simultaneously disentangle identity, expression, and illumination from the underlying rigid geometry, and it must do so relative to a fixed coordinate system that is never explicitly provided at test time. Unsurprisingly, these models tend to degrade for extreme poses, where training samples are scarce and the implicit anchor — effectively a neutral, frontal configuration embedded in the learned weights — lies far from the target.


We argue that relative head pose estimation offers a fundamentally easier formulation. Predicting the rigid transformation between two observed head configurations sidesteps the need for an implicit canonical frame and reduces the problem to estimating a displacement — a task that is both lower in intrinsic complexity and more amenable to domain transfer, since relative geometry is largely invariant to absolute coordinate conventions and appearance distribution shifts. This perspective also reveals a practical degree of freedom absent in absolute methods: the anchor can be chosen strategically at test time. In sequential settings such as video, a temporally close frame with known pose provides a natural anchor, keeping the relative rotation gap small and the prediction well within the model's comfort zone.


In this work we introduce VGGT-HPE, a 6DoF head pose estimator built on the Visual Geometry Grounded Transformer (VGGT), a large-scale geometry foundation model pre-trained for general-purpose camera pose and 3D reconstruction. We fine-tune VGGT with LoRA on synthetic two-view head pairs rendered from FLAME, supervising relative translation, rotation, and field of view in a compact geometric encoding. At test time, we compose the predicted relative pose with a known anchor pose to recover the absolute target pose in any desired coordinate frame. We evaluate on the BIWI benchmark within a unified pipeline that includes 6DRepNet and 6DoF Face as baselines, and provide a systematic analysis of how prediction error scales with the anchor–target rotation gap — directly validating the relative-is-easier hypothesis. Our contributions are as follows: ...

\section{Related Work}
\textbf{Monocular Head Pose Estimation.} Early head pose estimation methods relied on facial landmarks and 3D model fitting, typically recovering pose through geometric alignment or PnP-style optimization. More recent learning-based approaches instead regress pose directly from a face crop. HopeNet introduced a combined classification-and-regression strategy for Euler-angle prediction, showing that direct image-to-pose learning can be competitive without explicit landmark fitting. Subsequent works improved robustness to wider pose ranges and better rotation representations. WHENet targeted wide-range yaw estimation with a lightweight design suitable for real-time use, while 6DRepNet replaced Euler-angle regression with a continuous 6D rotation representation and a geodesic loss, improving stability under large rotations. Transformer-based methods such as TokenHPE further demonstrated that richer relational modeling over facial appearance can improve monocular head pose estimation. More recent 6DoF methods, including TRG, also incorporate facial geometry explicitly in order to improve translation and full pose prediction. Despite these differences, the dominant paradigm remains the same: a single image is mapped directly to an absolute pose defined in a dataset-specific canonical frame. As a result, the network must implicitly learn both the rigid orientation and the hidden reference frame relative to which that orientation is expressed.

\noindent\textbf{Relative Pose Formulations and Geometric Composition.} Relative pose estimation is a standard formulation in multiview geometry, visual odometry, and camera localization, where predicting the transformation between two observations is often easier than regressing a pose in a global frame. Compared with absolute regression, relative formulations reduce dependence on an externally fixed canonical coordinate system and focus the model on local geometric displacement. In head pose estimation, however, most learning-based methods still operate in the absolute monocular regime, and temporal or multi-frame information is more often used for smoothing, tracking, or feature aggregation than for explicit relative pose prediction followed by geometric composition. Our work takes the latter view. We predict the rigid transformation between an anchor frame and a target frame, then compose it with the known anchor pose to recover the target pose. This formulation is particularly attractive in video or multi-view settings, where the anchor can be chosen strategically, for example as a near-neutral or temporally adjacent frame, so that the relative rotation gap remains small. In this sense, our method connects head pose estimation more directly to classical relative geometry while preserving the convenience of feed-forward inference.

\noindent\textbf{Geometry Foundation Models for Pose Estimation.} Recent progress in 3D vision has shifted from narrowly task-specific models toward foundation models that jointly infer multiple geometric attributes such as camera parameters, depth, correspondences, and scene structure. VGGT is a representative example of this trend: a large feed-forward transformer pretrained for general visual geometry, including camera pose estimation, depth prediction, point maps, and point tracking across one or many views. Unlike conventional head pose estimators, which are trained specifically on facial crops and pose labels, VGGT learns broad geometric priors from generic multiview data. Our method builds on this observation. Rather than training a head-pose model from scratch, we adapt VGGT to the head domain with lightweight LoRA finetuning on synthetic FLAME renderings and repurpose its camera-pose machinery for relative 6DoF head pose estimation. This places our approach at the intersection of specialized head pose estimation and general-purpose geometric reasoning: the model inherits a strong prior for multiview structure while being specialized to the facial setting.

\section{Methodology}

\section{Experiments}

\begin{table}[t]
  \caption{Synthetic evaluation. Overall rotation errors (degrees), sorted by decreasing MAE. Lower is better. Best results are shown in \textbf{bold}, and second-best results are \underline{underlined}.}
  \label{tab:synthetic_final}
  \centering
  \small
  \setlength{\tabcolsep}{4pt}
  \begin{tabular}{@{}lcccc@{}}
    \toprule
    Method & Yaw $\downarrow$ & Pitch $\downarrow$ & Roll $\downarrow$ & MAE $\downarrow$ \\
    \midrule
    Small-Gap     & 17.03 & 23.20 & 21.77 & 20.66 \\
    Abs. Pair     & 3.12  & 4.59  & 7.01  & 4.91  \\
    T-Aux, No FoV & 2.94  & 5.45  & 6.01  & 4.80  \\
    VGGT-HPE      & 2.46  & 4.65  & 4.51  & 3.87  \\
    T-Aux         & 2.43  & 4.37  & 4.48  & 3.76  \\
    Rot.-Only     & 2.40  & 4.31  & 4.06  & 3.59  \\
    No FoV        & 2.39  & 4.13  & 4.19  & 3.57  \\
    Baseline      & \textbf{2.19} & 4.15 & 3.96 & 3.43 \\
    Geo Loss      & \underline{2.28} & \textbf{3.99} & \underline{3.76} & \underline{3.34} \\
    Abs. Single   & 2.44  & \underline{4.03} & \textbf{3.24} & \textbf{3.24} \\
    \bottomrule
  \end{tabular}
\end{table}

\begin{table}[t]
  \caption{BIWI evaluation. Overall rotation errors (degrees), sorted by decreasing MAE. Lower is better. Best results are shown in \textbf{bold}, and second-best results are \underline{underlined}.}
  \label{tab:biwi_final}
  \centering
  \small
  \setlength{\tabcolsep}{4pt}
  \begin{tabular}{@{}lcccc@{}}
    \toprule
    Method & Yaw $\downarrow$ & Pitch $\downarrow$ & Roll $\downarrow$ & MAE $\downarrow$ \\
    \midrule
    Small-Gap     & 7.38  & 7.07  & 3.88  & 6.11 \\
    Abs. Pair     & 3.61  & 6.99  & 6.49  & 5.69 \\
    Abs. Single   & 4.90  & 7.01  & 3.53  & 5.15 \\
    T-Aux, No FoV & 2.94  & 3.91  & 3.90  & 3.59 \\
    No FoV        & 2.64  & 4.05  & 3.61  & 3.43 \\
    T-Aux         & 2.76  & \underline{3.10} & 3.90 & 3.25 \\
    Geo Loss      & 2.95  & 3.24  & 3.32  & 3.17 \\
    Rot.-Only     & \underline{2.58} & 3.48 & 3.32 & 3.12 \\
    Baseline      & 2.61  & 3.17  & \underline{3.31} & \underline{3.03} \\
    VGGT-HPE      & \textbf{2.24} & \textbf{3.04} & \textbf{3.17} & \textbf{2.82} \\
    \bottomrule
  \end{tabular}
\end{table}

\begin{table*}[t]
  \caption{BIWI hard-pair benchmark on 360 neutral-anchor / extreme-query pairs. Lower is better. Best results are shown in \textbf{bold}, and second-best results are \underline{underlined}. `--` indicates that translation is not available for that method in this comparison.}
  \label{tab:biwi_hardpairs360}
  \centering
  \small
  \setlength{\tabcolsep}{5pt}
  \begin{tabular}{@{}lcccccccc@{}}
    \toprule
    & \multicolumn{4}{c}{Rotation Error (deg)} & \multicolumn{4}{c}{Translation Error (mm)} \\
    \cmidrule(lr){2-5} \cmidrule(lr){6-9}
    Method & Yaw & Pitch & Roll & MAE & Tx & Ty & Tz & L2 \\
    \midrule
    VGGT-HPE-Abs   & 40.74 & \underline{18.65} & 33.66 & 31.02 & \underline{46.09} & 86.15 & \underline{121.30} & \underline{167.84} \\
    TokenHPE       & 21.85 & 26.35             & 19.34 & 22.51 & --                  & --    & --                  & --                  \\
    TRG            & \underline{8.95} & 33.88 & 8.87  & 17.23 & \textbf{28.45}      & \underline{47.79} & 311.91 & 318.90 \\
    6DRepNet       & 14.27 & 18.91             & \textbf{6.81} & \underline{13.33} & -- & -- & -- & -- \\
    VGGT-HPE (Rel.)& \textbf{3.81} & \textbf{15.87} & \underline{6.93} & \textbf{8.87} & 63.65 & \textbf{34.10} & \textbf{118.47} & \textbf{150.50} \\
    \bottomrule
  \end{tabular}
\end{table*}

\begin{table*}[t]
  \caption{BIWI hard-pair benchmark on 360 neutral-anchor / extreme-query pairs. We additionally report MAE on the easier and harder 120-pair robustness subsets obtained by taking the bottom-5 and top-5 subject-wise pairwise rotation gaps from the original 15 pairs per subject. Lower is better. Best results are shown in \textbf{bold}, and second-best results are \underline{underlined}. `--` indicates that translation is not available for that method in this comparison.}
  \label{tab:biwi_hardpairs360_robust}
  \centering
  \small
  \setlength{\tabcolsep}{4pt}
  \begin{tabular}{@{}lcccccccccc@{}}
    \toprule
    & \multicolumn{4}{c}{Rotation Error (deg)} & \multicolumn{4}{c}{Translation Error (mm)} & \multicolumn{2}{c}{Robustness (MAE, deg)} \\
    \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-11}
    Method & Yaw & Pitch & Roll & MAE & Tx & Ty & Tz & L2 & Easy MAE & Hard MAE \\
    \midrule
    VGGT-HPE-Abs    & 40.74 & \underline{18.65} & 33.66 & 31.02 & \underline{46.09} & 86.15 & \underline{121.30} & \underline{167.84} & 30.99 & 30.56 \\
    TokenHPE        & 21.85 & 26.35             & 19.34 & 22.51 & --                  & --    & --                  & --                  & 21.84 & 24.66 \\
    TRG             & \underline{8.95} & 33.88 & 8.87  & 17.23 & \textbf{28.45}      & \underline{47.79} & 311.91 & 318.90 & 19.00 & 18.51 \\
    6DRepNet        & 14.27 & 18.91             & \textbf{6.81} & \underline{13.33} & -- & -- & -- & -- & \underline{12.85} & \underline{13.07} \\
    VGGT-HPE (Rel.) & \textbf{3.81} & \textbf{15.87} & \underline{6.93} & \textbf{8.87} & 63.65 & \textbf{34.10} & \textbf{118.47} & \textbf{150.50} & \textbf{8.47} & \textbf{9.49} \\
    \bottomrule
  \end{tabular}
\end{table*}


\begin{table*}[t]
  \caption{Synthetic hard-pair benchmark on 300 neutral-anchor / extreme-query FLAME validation pairs. We additionally report Euler MAE on the easier and harder 100-pair robustness subsets obtained by taking the bottom-5 and top-5 pairwise rotation gaps within each original 15-pair group. Lower is better. Best results are shown in \textbf{bold}.}
  \label{tab:flame_hardpairs300}
  \centering
  \small
  \setlength{\tabcolsep}{4pt}
  \begin{tabular}{@{}lcccccccccc@{}}
    \toprule
    & \multicolumn{4}{c}{Rotation Error (deg)} & \multicolumn{4}{c}{Translation Error (mm)} & \multicolumn{2}{c}{Robustness (Euler MAE, deg)} \\
    \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-11}
    Method & Yaw & Pitch & Roll & Euler MAE & Tx & Ty & Tz & L2 & Easy MAE & Hard MAE \\
    \midrule
    VGGT-HPE-Abs    & 3.28 & 5.08 & 4.57 & 4.31 & \textbf{2.94} & \textbf{2.90} & \textbf{9.63} & \textbf{11.62} & 3.44 & 5.94 \\
    VGGT-HPE (Rel.) & \textbf{2.88} & \textbf{4.84} & \textbf{4.24} & \textbf{3.98} & 34.64 & 34.42 & 36.78 & 70.07 & \textbf{2.07} & \textbf{6.80} \\
    \bottomrule
  \end{tabular}
\end{table*}

\begin{table*}[t]
  \caption{BIWI easiest neutral-anchor subset (`easy 4--8`, 360 pairs). Anchor mean: 4.01$^\circ$, query mean: 5.47$^\circ$, pair delta mean: 3.82$^\circ$. Lower is better. Best results are shown in \textbf{bold}.}
  \label{tab:biwi_easiest48}
  \centering
  \small
  \setlength{\tabcolsep}{4pt}
  \begin{tabular}{@{}lcccccccc@{}}
    \toprule
    & \multicolumn{4}{c}{Rotation Error (deg)} & \multicolumn{4}{c}{Translation Error (mm)} \\
    \cmidrule(lr){2-5} \cmidrule(lr){6-9}
    Method & Yaw & Pitch & Roll & MAE & Tx & Ty & Tz & L2 \\
    \midrule
    VGGT-HPE-Abs    & 4.02 & 2.26 & 1.52 & 2.60 & 53.18 & 91.97 & 118.74 & 181.99 \\
    VGGT-HPE (Rel.) & \textbf{1.17} & \textbf{0.74} & \textbf{0.97} & \textbf{0.96} & \textbf{20.55} & \textbf{6.74} & \textbf{15.40} & \textbf{28.73} \\
    \bottomrule
  \end{tabular}
\end{table*}

\begin{table*}[t]
  \caption{BIWI easy neutral-anchor benchmark. Main columns report the easiest subset (`4--8`, 360 pairs; anchor mean: 4.01$^\circ$, query mean: 5.47$^\circ$, pair delta mean: 3.82$^\circ$). The last two columns report MAE on progressively harder easy companion subsets `9--13` (query mean: 6.72$^\circ$, pair delta mean: 5.72$^\circ$) and `14--18` (query mean: 7.68$^\circ$, pair delta mean: 6.81$^\circ$). Lower is better. Best results are shown in \textbf{bold}, and second-best results are \underline{underlined}. `--` indicates that translation is not available for that method in this comparison.}
  \label{tab:biwi_easy_companions}
  \centering
  \small
  \setlength{\tabcolsep}{4pt}
  \begin{tabular}{@{}lcccccccccc@{}}
    \toprule
    & \multicolumn{4}{c}{Rotation Error (deg)} & \multicolumn{4}{c}{Translation Error (mm)} & \multicolumn{2}{c}{Companion MAE (deg)} \\
    \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-11}
    Method & Yaw & Pitch & Roll & MAE & Tx & Ty & Tz & L2 & 9--13 & 14--18 \\
    \midrule
    VGGT-HPE-Abs    & 5.62 & \underline{2.26} & 4.06 & 3.98 & 53.18 & 91.97 & 118.74 & 181.99 & \underline{2.92} & 2.99 \\
    TokenHPE        & 3.41 & 5.99            & 1.43 & 3.61 & --    & --    & --     & --     & 3.70 & 3.65 \\
    TRG             & 3.59 & 4.24            & 2.52 & 3.45 & \textbf{5.36} & \underline{16.06} & \underline{118.21} & \underline{119.85} & 3.36 & 3.49 \\
    6DRepNet        & \underline{2.31} & 4.93 & \underline{1.14} & \underline{2.80} & -- & -- & -- & -- & 2.98 & \underline{2.89} \\
    VGGT-HPE (Rel.) & \textbf{1.17} & \textbf{0.74} & \textbf{0.97} & \textbf{0.96} & \underline{20.55} & \textbf{6.74} & \textbf{15.40} & \textbf{28.73} & \textbf{1.21} & \textbf{1.32} \\
    \bottomrule
  \end{tabular}
\end{table*}

\begin{table*}[t]
  \caption{Synthetic easy frontal-anchor benchmark using the corrected canonical frontal H2C reference. Main columns report the easiest subset (`4--8`, 300 pairs; anchor mean: 16.23$^\circ$, query mean: 24.75$^\circ$, pair delta mean: 28.26$^\circ$). The last two columns report Euler MAE on progressively harder easy companion subsets `9--13` (query mean: 32.48$^\circ$, pair delta mean: 35.26$^\circ$) and `14--18` (query mean: 37.71$^\circ$, pair delta mean: 41.13$^\circ$). Lower is better. Best results are shown in \textbf{bold}.}
  \label{tab:flame_easy_companions}
  \centering
  \small
  \setlength{\tabcolsep}{4pt}
  \begin{tabular}{@{}lcccccccccc@{}}
    \toprule
    & \multicolumn{4}{c}{Rotation Error (deg)} & \multicolumn{4}{c}{Translation Error (mm)} & \multicolumn{2}{c}{Companion Euler MAE (deg)} \\
    \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-11}
    Method & Yaw & Pitch & Roll & Euler MAE & Tx & Ty & Tz & L2 & 9--13 & 14--18 \\
    \midrule
    VGGT-HPE-Abs    & 1.73 & 2.70 & 1.36 & 1.93 & \textbf{3.14} & \textbf{3.20} & \textbf{2.67} & \textbf{5.99} & 2.13 & 2.26 \\
    VGGT-HPE (Rel.) & \textbf{1.39} & \textbf{1.18} & \textbf{1.35} & \textbf{1.30} & 24.23 & 19.75 & 12.69 & 38.37 & \textbf{1.67} & \textbf{1.81} \\
    \bottomrule
  \end{tabular}
\end{table*}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.95\linewidth]{sec/fig/biwi_neutral_anchor_delta_compare.png}
  \caption{BIWI neutral-anchor $5^\circ$ bin sweep. VGGT-HPE remains the strongest method across all balanced bins, and its error increases more gradually with anchor-query rotation gap than the absolute variant and the monocular baselines.}
  \label{fig:biwi_neutral_anchor_sweep}
\end{figure}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.95\linewidth]{sec/fig/flame_frontal_anchor_delta_sweep.png}
  \caption{Synthetic frontal-anchor $5^\circ$ bin sweep. Using anchors close to the corrected frontal reference, VGGT-HPE consistently outperforms the absolute variant across the balanced bins as the anchor-query rotation gap increases.}
  \label{fig:flame_frontal_anchor_sweep}
\end{figure}



% Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
% This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets the figure captions and references in a smaller font.
The reason why such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The review process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in 11 pages.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler that should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use the options of \texttt{cvpr.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Use fractional references (\eg, this line is $087.5$), although in most cases the approximate location would be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please, number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for the reader to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean that some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not mean that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper, we present a performance analysis of our previous paper [1], and show that it is inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper, we present a performance analysis of the paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time that covers similar or overlapping material, you may need to refer to that submission to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, do not assume that the reviewers will read this material.

Sometimes your paper is about a problem that you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think that it is likely that the new article was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
However, for your results, you should not identify yourself and should not mention your participation in the challenge.
Instead, present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison with other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has only two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}


==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
The columns should be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered, and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

The captions of the figures and tables should be in 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centered.  Table captions should be above tables, while figure captions should be below figures.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period, and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use the footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example, at the beginning of the sentence, you can use
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, include the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When citing multiple papers at once, make sure that you cite them in numerical order such as this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \caption{Results.   Ours is better.}
  \label{tab:example}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead, use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise and, therefore, must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it is almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence, avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.
